Failure Detection and Isolation in Integrator Networks

Detection and isolation of link failures under the Laplacian consensus dynamics have been the focus of our previous study. Our results relate the failure of links in the network to jump discontinuities in the derivatives of the output responses of the nodes and exploit that relation to propose failure detection and isolation (FDI) techniques, accordingly. In this work, we extend the results to general linear networked dynamics. In particular, we show that with additional niceties of the integrator networks and the enhanced proofs, we are able to incorporate both unidirectional and bidirectional link failures. At the next step, we extend the available FDI techniques to accommodate the cases of bidirectional link failures and undirected topologies. Computer experiments with large networks and both directed and undirected topologies provide interesting insights as to the role of directionality, as well as the scalability of the proposed FDI techniques with the network size.

==> droppedFromIntro.tex <==
Linear agreement protocol has been extensively investigated in the recent literature as a fundamental evolution law for multi-agent networks, using probabilistic and deterministic models \cite{ConsensusOlfatiTAC2004,Tsitsiklis2009,RenBeard2005,RenBeard2008,Jad2008randomAgreement,BoydKim}. Earlier results on adjacency-based agreement rules can be traced back to Vicsek's model \cite{VicsekModel}. The present work is related to that in \cite{Yoon:2011:TFR:2286661.2286741}, in which Yoon and Tsumura calculate the single-input single-output transfer functions between pairs of nodes acting as the control input and measurement nodes for cyclic consensus systems. They also point out the interesting implications of the length of the shortest path between the input and measurement nodes on the stability margins and the relative degree of the calculated transfer functions. 
In  \cite{6161047}, Briegel et al. explore the connections between the relative degree and gain factor of the transfer function of a consensus network with an observer node (output) and a controller node (input) to the length and number of shortest paths between those two nodes.  %However, the proof Briegel et al. provide is flawed by their Lemma 3.1, where they make use of a matrix product commutative property that does not hold true. 

==> smallworld.tex <==
\subsection{Watts-Strogatz Small-World Graphs}\label{smallWorld}

In Watts-Strogatz small-world random graph model one starts with a circulant graph on a set of nodes labeled from $1$ to $n$, where for all $\{r,q\}\subset\mathbb{N}_n$, $r \neq q$, $r$ is connected to $q$ if, and only if, $|r-q|\leqslant\frac{d}{2}$ for a fixed $d$, which is an even degree parameter of the modeling. In other words, every node of the graph is connected to $\frac{d}{2}$ nodes immediately before and after it. Fig. \ref{fig:startCirculant} depicts one such graph for $n = 10$ and $d = 4$. 

\begin{figure}[H]
\centering
\subfigure[]{
\includegraphics[width = 0.21\textwidth]{circulant1.eps}
\label{fig:startCirculant}
}
\subfigure[]{
\includegraphics[width = 0.21\textwidth]{rewired1.eps}
\label{fig:rewired}
}
\label{fig:smallworldRandomProcess}
\caption{An instance of a Watts-Strogatz small-world random graph is depicted in \subref{fig:rewired}. This random instance is obtained from the graph in \subref{fig:startCirculant}, following the random rewiring process that preserves the cardinality of the edge-set.}
\end{figure}

Next, for every vertex $q \in \mathbb{N}_n$ and an edge incident to $q$, with probability $p$ this edge is replaced with another edge that is incident to $q$ but is non-existent in the original graph. The newly added edge is chosen uniformly and randomly amongst all edges that are incident to $q$ but are nonexistent in the original graph. Following this process, a randomly rewired version of the original circulant graph is obtained, of which one instance is depicted in Fig.~\ref{fig:rewired}.

In the following the aforementioned model parameters, size $n$, degree $d$, and rewiring probability $p$, are all varied and their effect on the cardinality of the detection sets as well as the required order of derivatives is investigated. The results are plotted in Fig. 13, where the sample means and standard variations are computed over $50$ instances. As with the case of Erd\H{o}s-R\'{e}nyi random graphs, the number of observation points and order of derivatives increase at a reasonable rate with the increasing network size. The results, in general, exhibit more variations as compared to the Erd\H{o}s-R\'{e}nyi random graphs, which can be attributed to the underlying random graph processes. It is worth highlighting that the cardinality of the detection set seems to be rather insensitive to the rewiring probability $p$ or the degree $d$, whereas the required order of derivatives is decreasing in the both parameters.


\begin{figure*}%[H]
\centering
\subfigure[The degree parameter is fixed at $4$.]{
\includegraphics[width = 0.3\textwidth]{smallworldNumberVersusSize.eps}
\label{fig:1}
}
\subfigure[The degree parameter is fixed at $4$.]{
\includegraphics[width = 0.3\textwidth]{smallworldOrderVersusSize.eps}
\label{fig:2}
}
\subfigure[The degree parameter is fixed at $4$.]{
\includegraphics[width = 0.3\textwidth]{smallworldNumberVersusProbability.eps}
\label{fig:3}
}
\subfigure[The degree parameter is fixed at $4$.]{
\includegraphics[width = 0.3\textwidth]{smallworldOrderVersusProbability.eps}
\label{fig:4}
}
\subfigure[The rewiring probability is fixed at $0.21$.]{
\includegraphics[width = 0.3\textwidth]{smallworldNumberVersusDegree.eps}
\label{fig:5}
}
\subfigure[The rewiring probability is fixed at $0.21$.]{
\includegraphics[width = 0.3\textwidth]{smallworldOrderVersusDegree.eps}
\label{fig:6}
}
\label{fig:smallworldBooogh}
\caption{Simulation Results for Watts-Strogatz Small-World Random Graph Model}
\end{figure*}
